An Investigation into Protestware

Protests are public expressions of personal or collective discontent with the current state of affairs. Although traditional protests involve in-person events, the ubiquity of computers and software opened up a new avenue for activism: protestware. The roots of protestware date back to the early days of computing. However, recent events in the Russo-Ukrainian war has sparked a new wave of protestware. While news and media are heavily reporting on individual protestware as they are discovered, the understanding of such software as a whole is severely limited. In particular, we do not have a detailed understanding of their characteristics and their impact on the community. To address this gap, we first collect 32 samples of protestware. Then, with these samples, we formulate characteristics of protestware using inductive analysis. In addition, we analyze the aftermath of the protestware which has potential to affect the software supply chain in terms of community sentiment and usage. We report that: (1) protestware has three notable characteristics, namely, i) the "nature of inducing protest" is diverse, ii) the "nature of targeting users" is discriminatory, and iii) the "nature of transparency" is not always respected; (2) disruptive protestware may cause substantial adverse impact on downstream users; (3) developers of protestware may not shift their beliefs even with pushback; (4) the usage of protestware from JavaScript libraries has been seen to generally increase over time.

==> correlation-rq1__removed_.tex <==
%Include the dependencies look or not, since WayBack machine didn't give any good snapshots before 2024. (should we include what we did and saw in a few repos?)

\subsection{Analyzing correlations}
\JC{TODO.} %Talk about active or not 
% We then applied these categorizations manually to the dataset we were studying~\cite{dataset}, which included 16 known implementations of protestware in open source software and discarded one(Mistape WordPress plugin, which finds mistakes in text you typed) for lack of relevance, as it was a security issue instead of intentional protest. 
First, Figure ~\ref{fig:totalBar} shows how the protestware that was studied break down into our chosen categories. The green bars show how many of either malicious and benign were studied, showing that an equal number were analyzed. The blue bar indicates if they still remain or not. As it can be seen, slightly more 
% \JC{When reporting results in prose, we need to be precise. Say how many more exactly.} 
benign protestware(5) remained than the malicious(4). The red bar indicates if the protestware was meant as a targeted attack or not. The malicious protestware saw only targeted attacks. Since negative actions will occur from running their code, developers want to ensure that it only affects the people they want to protest against. 
% \TF{Should I mention that malicious universal is considered Malware by us, as it is already in the grouped bar chart caption} \JC{What you mean by ``malicious universal is considered Malware by us''.}
The yellow bars indicate whether the protestware behavior is easily visible to users typically written in a public file such as README. Both malicious and benign have low reporting scores of public visibility with 3 out of 8.
% \JC{The yellow bar seems equal for both mal and benign to me.}. %Correct, I forgot to change the text after updating the chart 
However, the benign cases, although the same, had less incentive to explain the changes, since many of them did not affect functionality, like changing an image or text. 


\begin{figure}[h] %Figure for the breakdown with taxonomy 
    \centering
    \includegraphics[width=\linewidth]{Figures/breakdownChart.png}
    \caption{ Grouped bar chart of protestware breakdowns by our characteristics. Initially separated by implementation.
    }
    \label{fig:totalBar}
\end{figure}

\begin{SummaryBox}{Takeaway: Heading.}
Summary text.
\end{SummaryBox}

==> discussion-backup.tex <==
\section{Discussion}

\subsection{Limitations}
\JC{Bias to towards recent events. We didn't find any protestware before 2010 I think?}
\JC{In case I forget, it is also possible that an author added a potential symptom without specifying it in the commit, which is a limitation of using commit history. This is especially concerning for symption 1, since it involves the source code and reviewing the source code manually in its entirety would be infeasible. This comment should go in the threats to validity or limitation section.}
\JC{Maybe split this into construct validity, internal validity, and external validity.}
With the unique nature of the attack vector, being a modification being made by the developer themselves, alongside the limited dataset currently available for analysis, the symptomology provided by this paper is in no way all-inclusive. Our simplified categorization scheme also led to a few limitations when putting examples into categories. The main issue is that the binary categories do not indicate a notion of severity with the effect. For example, a malicious code could be writing to a file with a protesting message as an example of a lesser degree of malicious intent versus deleting files on the users computer. Another issue is classification into categories because the category might not have a sharp division between sides. For example, the developer may have included comments in the commit about the functionality changing for particular users, but not in the description file like README. In which case, the protestware would have been marked as private \JC{We need to be consistent. Pick a cateogry name and stick to it. Originally, ``secret'' was used, but here we use ``private''. Personally, I prefer ``private'' over ``secret'', since we have ``public''.} because most users will roll forward the commits to update the project without looking at the commit messages, but a description in the README file, no matter how well hidden, is still possibly alerting the user that pays attention to the changes in functionality from there. \JC{I actually don't think this is a grey area, and therefore is not a limitation. If your definition of ``public'' is that it must appear in the README file, then we can confidently say it's ``private'' if it's not in the README file but in the commit. Unless of course you think your definitions are not good to begin with, which is another threat altogether.}

The framework \JC{Which framework?} is also language agnostic, which means that each coding language will need to be evaluated under the same set of criteria, which might be different given the data constructs within various languages. Another limitation may be that our work primarily focuses on what has changed in the open source code to turn it into protestware. If the protestware existed before the change you are currently examining then it would not be detected\JC{Why not? Please clarify.}. However, you could simply apply the framework iteratively through all the previous commit changes to see if any of them detect protestware. The only problem with this is that it will most likely be slow, especially with a huge code base. The final limitation is that provided any set of symptoms, a smart developer can think of ways around them by nesting functionality inside normal code. For example, if the developer already had an accessibility feature in their code for people from Russia, then all they need to do is alter that feature to have slightly different functionality, like a rejection of service or they can nest the changed code into their servers, which may be accessed by their open source code \JC{Can we get a citation for this. It doesn't have to be for protestware specifically, it just need to be about ways to hide features etc.}. 
\JC{Another threat to validity is commit messages may not reflect everything done, \ie you will have false negatives. A commit message can also be untruthful. Did you verify that each commit was what it claimed to be?}

\subsection{Applications/ Future Work}
Although we did not have enough time to investigate the usefulness of detecting and applying our set of symptoms to a chosen dataset, we did come up with a few ideas on how one might apply our framework. The first is to identify a targeted action of symptom ~\ref{symptom:targetLocation}. When a conditional if statement is applied to only a set of users that is not addressed for the remaining set of users. One would need to first identify the set that is being conditioned upon and determine how small that set is compared to the total set of users, presumably have other accessibility functions for the set of all users. This task might be performed with backward slicing (refer ~\cite{AutomaticUncover}) of conditional if statements that redirect the behavior of execution only for a subset of users without accounting for other users using constructs like a switch statement or chains of if else statements depending on the language. 

The use of an LLM was proposed because of their effective analysis of text and code. Previous work has applied LLM's to detecting emotion within text and adding or adjusting code such as Github's copilot. Utilizing tools like these seem to provide an effective solution to detecting Symptoms ~\ref{symptom:aggressiveLanguage} and ~\ref{symptom:additionalLanguage} because due to the emotion nature of protest, the aggressive language toward a group of people seems to be identifiable and also the language of the developer compared to text used should also be simple to detect. 

The final symptom, number ~\ref{symptom:benign}, should be easier to detect as it is checking if important text or images in the project have changed. The next test would be to identify the text as having a political or protest meaning behind them. For images this might include image identification if it includes images important to politics such as flags or symbols. alternatively the image may have political text within it, which would require image text classification potentially using optical character recognition on the changed image. 

==> intro-backup.tex <==
\section{Introduction}

% \JC{Some devs do sanctioning or complete removal of their software in act of protest, but this isn't really protestware. What if this study was extended to include any type of protesting in software industry?}
% \JC{Perhaps study how the protests affected the software supply chain with case studies, how many software relies on them, etc?}
%The difference analysis might be done by Sazz or Sathvik if possible
% \JC{RQ: What do developers think of protestware? Can be done via study or looking for comments online. What is the line between accceptable and not-acceptable protestware? Do you think protestware or in-person protests are more xyz?}

Protest is a deeply ingrained form of expression in which individuals voice their dissatisfaction with societal issues, either personal or collective, typically through marches and rallies, hoping to inspire others to join their cause. 
Yet, in our digital era, where technology intricately weaves into our daily lives, the essence of protest has evolved. Now, programmers wield a unique form of expression, not through banners or chants, but through the very code they craft. This novel concept, often termed as 'protestware', embodies a fusion of activism and technology, reshaping how we perceive and participate in modern dissent.
% The issues when dealing with protestware are the widespread effect it might have and the lack of methods to classify and identify these potentially harmful software.
%GPT Fixing


The challenges associated with protestware include its potential for widespread impact and the absence of effective methods to classify and identify such potentially harmful software. 
%Importance:
The impact can be seen when one looks at the utilization of third-party libraries and repositories in the software industry. Having such dependencies is helpful for developers as it eliminates the need to create all aspects of said projects from scratch. Open source software (OSS) is a subset of said libraries and repositories that are able to be freely modified and implemented into other projects, creating a community-developed set of tools that can be utilized by any developer for any purpose without restriction ~\cite{OSS}. 
% OSS developers can turn their software into protestware as they are not contractually obligated to implement anything specific. 
Though this creates a convenience within the development ecosystem, it has also spawned attack vectors for individuals, as a form of protest, to potentially affect many that use their developed code.  
% Protestware, an attack vector more prevalent in recent history, is an instance of the abuse of open source software that can impact its user base at a mass scale\JC{Any claim made should be cited. Also, don't define something with a general definition. Be more specific and say directly what protestware is.}.
Through direct alteration by the developer, any and all members of the supply chain that rely on that original project will in turn be effected, with the potential for severe damage being present. Unlike typical supply chain attacks, where the attacker needs to infiltrate one of the dependencies to gain access to the larger system, the dependency is altered by the original, trusted developer. 

Additionally, software can assist in inducing protest among like minded individuals not necessarily through the code they write but also software written to aid other types of protests as well. 
% Along with this, the potentially sporadic and unpredictable nature of how a developer would change their code (as it can be for any type of protest with varying levels of obfuscation), makes the current systems for malware detection less effective. This is especially true as a standard system of identification and categorization has yet to be established for it.
%What this paper does

Therefore, this paper aims to provide a useful taxonomy and analysis of protestware by looking at known instances of software which directly induce protest. Specifically, in this paper we address the following research questions.

\begin{itemize}
    \item \textbf{RQ1:} What are the prominent characteristics of protestware?
    \item \textbf{RQ2:} What protestware still exist and how did the software with altered code affect the user base? 
\end{itemize}

\input{tables/general-all}

%The summary of the table and interesting finds
Table ~\ref{tab:allProtestware} shows an overview of our results from both \textbf{RQ}'s as it pertains to each of the protestware collected. Each of the 31 protestware studied have a row to indicate the attributes determined for the Basic Specifications, characteristics(\textbf{RQ1}), and if the protestware code still exists within the repository(\textbf{RQ2}). It can be seen from the table that there is variety in the function of protestware, some handling visual content like colors and alerts while other handle voice bots, calculations, or locations. Many of them are web based implementations (using JavaScript or TypeScript) and the ones with altered software are more likely to be a library. 
% For our symptoms, we see a strong coverage over the relevent software, some protestware are not marked for reasons based on the implementation type as described later. Especially our 5th symptom, was seen with more coverage than others. %No longer doing symptoms




% the attack type, and utilize these findings to construct a set of potential indicators for use in future detection projects.
% \JC{I find the sentences to be too long very often.}

% {\bf Solution sketch:} First off, we will do a thorough literature review to understand what has been done to analyze this sort of software. Any information we gain from there, we utilize to further refine our questions. We could then be able to use grounded theory to make categories for the protestware by analyzing particular properties of the code, execution, and assumptions and repeating the cycle to figure out the categories to use. Finally, we will analyze this information using either data visualization to assist in finding predictive patterns or brute force to look at all our examples to figure out a possible solutions for particular categories. The feasibility of these tasks is sound. A possible drawback which may exist is finding a limited number of protestwares to study. If this is the case, we will learn more detailed information from each protestware, and describe additional possibilities that could exist beyond what was seen. 
% % Should write about the feasibility of solving this problem. Also, how do you plan to solve it?

% {\bf Challenges:} Some challenges we may encounter are having only a limited dataset, identifying coherent categories, and gathering additional information from reverted repositories. So far, we have found one dataset on github that has approximately less than 30 entries, but some links offer additional information such as dependencies of a package being imported or specific malicious code. Figuring out a good categorization may also be difficult because there could be too many categories to be helpful or too few to generalize. So these categories will probably need to be adjusted as we go along. The final potential issue is accessing information that may have been deleted or reverted back because of public pressure. We believe there are ways around this as there should be information stored on the internet about saved, past websites.
% Write about the challenges you need to overcome to solve this problem.
% Not sure how we are supposed to know about the challenges before getting into the depth of the project. 



==> quotes.tex <==
Quotes by Protestware Authors(Developers)
\JC{We don't have enough for a seperate RQ. How can we incldue these into our current RQs? We also need to have a good reason for not interviewing people.}
\JC{1, 2, and 4 seems to be about making sure the Russian people gets proper info, since Russia is censoring them.}
\SR{I like this protestware-by-protesware lookup for news articles. Well done, Jesse! These are all good findings. Now, we will have to think about how we can integrate them seamlessly into the aftermath of RQ. Can you also please write about the methodology used to find these articles?}
\SR{Also, it will be nice to find something relevant to why people are still using these tools -- to explain their popularity.}
\JC{Unforunately, I didn't find anything on why they are still being used.}
\JC{I will organize smth with what I have and put it in the prose. PTAL \cref{sec:triggers} and \cref{sec:supplychaineffects}.}
\begin{enumerate}
    \item \textbf{styled-components:} 
    Cause: Evan Jacobs, one of the primary maintainers behind styled-components, told TechCrunch that his project has a history of activism, “most notably our support of the [Black Lives Matter] movement and recommendation to our users to consider donations to the Equal Justice Initiative.” He added: “I had heard that the Russian government was beginning to censor Western news websites and realized that we had a unique opportunity to deliver a concise, informative message via an atypical channel: our npm package installations.” 
    
    Jacobs felt it was crucial that Russians get accurate news about the war that is free from state interference. He modified styled-components, which had more than 15 million monthly downloads as of April, to display a bilingual message to Russia-based users summarizing the “many atrocities being committed by the Russian army in Ukraine.”
    
    “Did it make an impact? We’ll probably never know,” Jacobs said. “That being said, I think it was completely worth the chance to disseminate information and hopefully catch the eye of software folks in Russia that might not have seen what was happening otherwise.”~\cite{protestwareontherise}

    \item \textbf{es5-ext:}
    Cause: Another developer, Mariusz Nowak, the creator of the es5-ext project, modified later versions of the library to direct Russia and Belarus-based users to accurate news sources like the BBC’s Tor service. Nowak told TechCrunch about the decision to modify the code, saying it was because Russians “are not exactly sure what’s going on, and they’re under influence of their propaganda media,” referring to the strict state control over Russian media. “This message shows only if you install software in Russia, it’s not really visible for other parts of the world,” Nowak said. 
    
    Effect: Nowak said using his open source library for activism did not affect his credibility among the wider community, but he did receive a handful of angry responses at the beginning.~\cite{protestwareontherise}

    \item \textbf{peacenotwar:}
    ``This code serves as a non-destructive example of why controlling your node modules is important. It also serves as a non-violent protest against Russia's aggression that threatens the world right now.''~\cite{peacenotwar} 

    \item \textbf{event-source-polyfill:} Translated from Russian using Google Translate, the author says that Russian government is restricting citizens' access to external information by imposing one-sided formulations and versions of what is happening. He recommends using Tor browser and visit BBC's dark web mirror~\cite{eventsourcecommit}. 
    
    \item \textbf{left-pad:}  

    ``A few weeks ago a patent lawyer sent me an e-mail asking me to unpublish “kik” module from NPM. My answer was “no” and he replied me saying “I don’t wanna be dick about it, but “kik” is our registered brand and our lawyers gonna be banging on your door, and taking down your accounts.”
    
    When I started coding Kik, didn’t know there is a company with same name. And I didn’t want to let a company force me to change the name of it. After I refused them, they reached NPM’s support emphasizing their lawyer power in every single e-mail CC’ing me. @izs accepted to change the ownership of this module, without my permission.''~\cite{leftpadblogarchive}


    \item \textbf{faker (also applies to colors):}

    "Respectfully, I am no longer going to support Fortune 500s ( and other smaller sized companies ) with my free work. There isn't much else to say. Take this as an opportunity to send me a six figure yearly contract or fork the project and have someone else work on it."~\cite{fakerquotearchive}

   \item \textbf{node-ipc:}

   Aftermath: Vulnerable versions of node-ipc existed on npmjs registry for no more than 24 hours~\cite{nodeipcsnyk} and still have affected large OSS projects. For instance, Vue.js~\cite{vuejs}, a popular JavaScript front-end framework, always used the latest minor and patch versions of node-ipc instead of pinning a known safe version~\cite{nodeipcbleepingcomputer}. This would inevitably cause Vue.js to use a vulnerable version, though it has since been fixed~\cite{nodeipcsnyk}.
   

    
    
\end{enumerate}

Recommendations
\begin{enumerate}
    \item 
    “When it comes to this particular issue of trust, I believe the best way for it to be handled is with proper software supply chain hygiene,” Brian Fox, CTO of supply chain security firm Sonatype, tells CSO. “When you’re choosing what open-source projects to use, you need to look at the maintainers.”~\cite{developersabotages}
\end{enumerate}

Others
\begin{enumerate}
    \item  
    Feross Aboukhadijeh, a prolific open source maintainer and the founder of Socket, told TechCrunch in a recent call that development teams often put too much trust in open source code, which can be catastrophic if a deliberate vulnerability is introduced into the supply chain and goes unnoticed.~\cite{socketlands}
\end{enumerate}




==> relatedWorkOld.tex <==
\section{Related Work}
 


%Here we will talk about the work that is similar to ours in the nature of qualitatively looking at protestware or open source code and evaluating how to identify or %prevent attack vectors along open source software. 

%Divided it for proper understanding and clear view


In this section, we discuss about the prior research relevant to our investigation, focusing on the qualitative examinations of protestware and the open-source software, along with the efforts to identify and prevent potential attack within the open-source ecosystem.
\\

%A main contribution to our research is an unpublished paper titled "The Vulnerability of Open-source Software: Protestware." This introduced the concept of protestware and examines its implications for the security of open-source software. By telling gaps in existing research and offering an in-depth analysis, the paper shows the challenges posed by protestware. These insights guide our understanding of how protestware operates within open-source ecosystems and inform our strategies for enhancing the security of these projects. And our paper consists of all the details in some or the other way as mentioned in the above paper. %

 %"Ethical Considerations Towards Protestware" 
Mainly, the study referenced in ~\cite{Protestware} explores the ethical aspects of protestware within the open-source software (OSS) community. The paper examines the challenges of incorporating political messages in software libraries and suggests efforts to promote ethical responsibility among maintainers and contributors. These considerations are essential for our analysis of protestware attributes and detection frameworks, as they help us to understand the motivations behind protestware and the ethical dilemmas that it may pose. By integrating these ethical perspectives, our research aims to develop a more Systemic approach to identify and manage protestware in open-source environments, ensuring that software development adheres to ethical standards.

%"Always Contribute Back: A Qualitative Study on Security Challenges of the Open Source Supply Chain,"
Another relevant study, ~\cite{AlwaysContributeBack}, delves into the security challenges of Open Source Components (OSCs) in software development. This research Highlights the importance of understanding OSC utilization and decision-making processes within companies. These insights are particularly valuable for our study as they tell us on how organizations integrate and manage open-source software, which is frequently targeted by protestware. By understanding these dynamics, our research can better identify potential vulnerabilities and entry points within the ecosystem that protestware Takes advantage of. Furthermore, knowledge of how companies assess and integrate OSCs can inform the development of more effective detection frameworks, helping to Lessen the risks associated with these components and enhance the overall security against protestware within the open-source ecosystem.

%"Poster: Towards Using Source Code Repositories to Identify Software Supply Chain Attacks"
In the domain of detection methodologies,  ~\cite{TowardsUsing} proposes a method for detecting software supply chain attacks by analyzing code changes in repositories. This approach offers valuable insights into identifying potential malicious interventions within the software supply chain, complementing our investigation into protestware attributes and detection frameworks. While software supply chain attacks usually involve unauthorized modifications to software components that intend to compromise user security, protestware, although the similar one, specifically involves the insertion of politically or socially motivated code into open-source projects. Understanding the detection techniques for software supply chain attacks is beneficial for our study on protestware, as both involve unauthorized code alterations. By applying methodologies developed for detecting supply chain attacks, we can adapt and refine these techniques to specifically identify and reduce protestware intrusions, which may be more indirect or embedded in legitimate code updates, thereby enhancing the robustness of open-source ecosystems against such targeted threats.


%"Towards Detection of Software Supply Chain Attacks by Forensic Artifacts"
Similarly,  ~\cite{TowardsDetection} introduces Buildwatch, a tool for detecting malicious activities in the software supply chain. This automated monitoring capability contributes to enhancing software security by providing early detection and response mechanisms to potential threats, including those posed by protestware. This is particularly relevant to our research goals of analyzing code to detect malicious components. Although Buildwatch is mainly concerned with broader software supply chain vulnerabilities, its methods are especially relevant to our project because they can be customized to detect the complexities of protestware. By incorporating these detection techniques, our research is better equipped to identify and understand the distinctive signatures and behaviors of protestware, improving our ability to address its risks in open-source projects.

%"InputScope: Uncovering Secrets in Mobile Apps via User Input Validation Analysis"
%CryptoGuard: High Precision Detection of Cryptographic Vulnerabilities in Massive-sized Java Projects
Additionally, ~\cite{AutomaticUncover} introduces INPUTSCOPE, a tool designed to uncover concealed behaviors within mobile applications through static taint analysis. It underscores the critical role of input validation in ensuring app security, a principle that's helpful with our ongoing research on protestware elements to ensure what input commands can enable/shoot a protesware issue. By integrating insights from INPUTSCOPE, we can deepen our comprehension of software security challenges, particularly in the context of protestware. This integration will enhance the development of robust protestware detection frameworks by providing valuable perspectives on how malicious behaviors may be covered within app code.

Moreover, the paper ~\cite{Cryptogaurd} presents a static analysis tool specifically tailored for identifying cryptographic misuses in Java programs. This work is highly relevant to our research objectives as it highlights the importance of pinpointing security vulnerabilities. By leveraging advanced static analysis techniques, such as backward slicing, CryptoGuard achieves a high precision in detecting instances of improper cryptographic usage. This seamless alignment of backward slicing with our exploration of protestware elements and detection frameworks will offer good insights into the complexities of security vulnerabilities within the software supply chain.
Furthermore, integrating insights from CryptoGuard not only improves our understanding of security vulnerabilities but also significantly contributes to the enhancement of robust protestware detection mechanisms. By combining the methodologies of both INPUTSCOPE and CryptoGuard, our research endeavors to provide a thorough approach to detecting and mitigating protestware threats in software applications.

%"On DDoS Attacks as an Expression of Digital Protest in the Russo-Ukrainian War 2022"
Nevertheless, the paper ~\cite{DDoS} explores the examination of Distributed Denial of Service (DDoS) attacks, which are often used as a form of digital protest during geopolitical conflicts. While DDoS attacks primarily aim to interrupt the services by crushing them with traffic, protestware involves the incorporation of protest-driven functionalities within software, subtly or clearly altering its behavior to reflect political or social activism. This research is applicable to our study as it explores into the intersection of cyber activities, protests, and geopolitical events, providing a broader context for digital activism.
Understanding how DDoS attacks work helps us see the reasons behind them, how they're carried out, and their effects, and to compare these with the more hidden nature of protestware. This comparison gives us a deeper understanding of the different ways digital protests can appear and be noticed, improving our tools for analyzing protestware. By bringing this understanding into our study of protestware, we can more effectively identify and examine protest-driven cyber activities in open-source software environments, especially in terms of how different motivations and effects emerge based on the type of digital protest.

Moreover, recent incidents, including the purposeful introduction of corrupted versions into widely used repositories, have underscored the urgent need to tackle the issue of protestware within the open-source community. Our research draws on a range of sources to academic studies, blog posts, and firsthand observations from GitHub repositories to develop effective strategies for detecting and mitigating the protestware in the open-source environments. This thorough approach is designed to ensure that open-source software remains secure and trustworthy for users around the world. Ultimately, we aim to protect the integrity of open-source repositories and guard against the potential misuse of software for protest or other unauthorized modifications.






==> researchQuestions.tex <==
\section{Research Questions and Result Overview}
% \JC{I think we should define what you mean by ``component''. \eg is it a package, single file, or something else?}
% \quad \textbf{RQ1:} What is a simple and intuitive way to categorize protestware to enhance understanding?
% What are the components seen in the current corpus of protestware and are they indicative of this attack type being present within a given project?
% \JC{Does the second part mean you're trying to see which components in a protestware is a signal that it's a protestware?}


% Then, our symptoms have variable coverage of the protestware with symptoms 1 and 2 seemingly occurring more often together, along with symptoms 3 and 4 behaving similarly. Only one protestware (SweetAlert2) had all 4 symptoms.
% \SR{@Jesse or @Tanner, please write an overview of the findings.}\TF{Working on it}
% \textbf{RQ2:} What set of symptoms be generated for the purpose of detecting protestware in GitHub repositories?


% \JC{Define ``external factor'' and likewise ``internal factor'', or maybe rephrase the question. Also, define ``base project''. }


==> results-rq1-old.tex <==
\SR{Sazz to start revision from here.}

\section{RQ1: Types and Functionalities}
\SR{@Jesse, if you wake up earlier than I do, can you please clean this up by only keeping the language, type (i.e., library or standalone), and functionality? For the functionality, you can refer to the table, where we have the description of the functionalities.}
An examination of the data surrounding the protestware in terms of the utilized programming language and type, either standalone or library, was performed, allowing an understanding of what kind of project is more likely to be converted into protestware. 
% In order to compare these statistics at the time of insertion of protestware, we also used the Wayback Machine to find the closest snapshot to the insertion and then another one about a week to a month after, depending on the frequency of snapshots provided.



We performed analysis of the protestware type, primary programming language used, and functionality to answer \textbf{RQ1}. The most used programming language of each project was determined using GitHub's provided metrics of language percentage. The number of these primary languages seen are shown in Figure \ref{fig:language} with 22 of them being web-based languages like JavaScript, HTML, and PHP. Unsurprisingly, the functionality largely followed a similar pattern, with many being JavaScript libraries or contributions to web-based applications. Many of them relate to pop-up boxes or alerts for the user such as 'awesome-prometheus-alerts','SweetAlert2', and 'yad' which stands for Yet Another Dialog. Others relate to the visual or audio in other ways with 'RedisDesktopManager' being a GUI for a desktop application, 'Quake3e' being a game engine, and 'voicybot' being a voice bot for a cloud-based instant messaging service. 



% \begin{figure}
%     \centering
%     \begin{subfigure}{0.49\linewidth}
%       \center{\includegraphics[width=\linewidth]{Figures/aftermathChange1.png} }
%       \caption{} \label{fig:popularityStars1}
%     \end{subfigure}
%     \begin{subfigure}{0.49\linewidth}
%       \center{\includegraphics[width=\linewidth]{Figures/aftermathChange2.png}}
%       \caption{}\label{fig:popularityStars2}
%     \end{subfigure}
%     \begin{subfigure}{0.49\linewidth}
%       \center{\includegraphics[width=\linewidth]{Figures/aftermathWatching.png}}
%       \caption{}\label{fig:popularityStars2}
%     \end{subfigure}
%     \begin{subfigure}{0.49\linewidth}
%       \center{\includegraphics[width=\linewidth]{Figures/aftermathForks.png}}
%       \caption{}\label{fig:popularityForks}
%     \end{subfigure}
%     % \caption{Prototype Figure displaying star counts during Protestware insertion compared with now/ most recent of more popular software (>3000 stars)}
   
%     % \caption{Prototype Figure displaying star counts during Protestware insertion compared with now/ most recent of less popular software (<3000 stars) 
%     % }
%     % \caption{Chart looking at watching stats of all software}
%     \caption{Charts looking at popularity statistics on software}
% \end{figure}
%Turn these into a big table
% \TF{Could potentially include a graph of the resulting stats, (start time vs. full date). Developer or user interview(Need IRB)?  }
% \SR{Let's keep the interview part for a follow-up study. We can point this out in the discussion and conclusion as "future work"?}

% \TF{Additional analysis direction could be looking at longevity of how long the Protestware lasted and patterns.}
% \SR{Great idea!}

%which was a rarity and the only protestware with types benign, targeted, and public. 



% All 16 examples had at least one symptom and many had multiple symptoms. 

% Symptomology:
% Conditional statements examining language preference with small set of languages
% Conditional statements examining geographical location with small set of locations
% Language string in source code / project files that differs from the primary language 
% Implements known protestware
% Detecting Targeted Protestware:
% Detecting Universal Protestware: 


% {\bf Criteria for success:} As this is a qualitative study, our measure of success will depend on what can be learned from protestwares that have been developed in the past. The proposed solution should be ways to identify these protestwares given certain categories. The measure of success for these solutions should be the generalizability to handle cases which don't exist yet and coverage of the solutions to apply to any possible protestware given the scope of malicious or undesirable code in open source software projects. 
% % How would you measure the success of your project? Some of the evaluation criteria can be, i.e., runtime performance, accuracy, generalizability of the proposed solution, etc.

% {\bf Datasets:} The following dataset \cite{dataset} is a github repository containing a list of identified protestware in open source projects. We will use this dataset and the links provided to find additional information regarding the protestware and details about each instance. In this way, we will be generating our own dataset with information about each instance such as protestware type, where it was included, desired outcome, etc. The method for creating this dataset will be by hand as we will look individually through each of the protestwares that are cited in the list to determine the attributes. Attributes can be added or deleted when it's determined to be helpful to do so. The reason we are able to do this manually is that the dataset is fairly small. Additional datasets would be desired but unlikely to exist. 
% What dataset(s) will you use to conduct the experiments. If you want to create your own dataset, you need to write the method for dataset creation, too.


==> results-rq3-old.tex <==
% \section{RQ3: Symptoms}

% \label{sympt}
% \label{sympResults}
% \subsection{Definitions}
% Through our systematic inductive review, we found the following symptoms\footnote{
% While we produced the list of symptoms systematically, we acknowledge that it may not be exhaustive.}.

% \JC{Takeaway for each symptom? How would that work...hm...}
% \textbf{Isolation Filter.} \SR{Add counts from table 2?} A protestware has an isolation filter if it performs some form of check that isolates a particular group of users, such as location, IP, or language checking, with the resulting behavior not being broadly applied to all groups, therefore making it not an accessibility feature.
% For example, \cref{isofilt} shows a code snippet where code implementing a restriction based on a set of locations around Russia was added for es5-ext~\cite{esfiveextcommit}. 




% \textbf{Advocacy Communication.} 
% \label{sec:advocomm}
% A protestware has advocacy communication if it contains one or more files (\eg code, documentation, images) with a message containing aggressive language or ideology promotion. The communication may or may not require the software to be run to be seen.
% For instance, \cref{adcomm} shows a code snippet in awesome-prometheus-alerts with aggressive language against Russians~\cite{awesomeprometheusalertscommit}. 
% In addition, this code snippet is saved in a file called [Middle-finger-emoji].md.

% \textbf{Linguistic Alteration.} A protestware has linguistic alteration if the developer removes a previously supported language entirely or if the source code contains new string(s) in a language different from the primary language of the developer\footnote{Primary language is determined by the language of comments and text files like README.md. Also, the strings should not be used for translation purposes.}.
% An example is RedisDesktopManager, where a Russian translation file is removed~\cite{redisdesktopmanagercommit}, as shown in~\cref{redisnorustrans}.

% Removal of a previously supported language is a strong symptom of protest, while the addition of strings in a non-primary language alone may not necessary be indicative of protest. In case of adding non-primary language strings, it may be useful to check for advocacy communication. \JC{Now that I write this...it seems like then we don't even need ``new strings in a non-primary language'' to be a symptom since we will always need to check what all the strings in repo are saying, regardless of language? We also likely need to include possible combos of symps.}

\begin{figure}[H]
    \centering
    % \includegraphics[width=\linewidth]{Figures/ScreenshotSymptom3.png}
    \small 
    \begin{lstlisting}[style=base, 
        language=html, 
        label={redisnorustrans},
        caption={Example of linguistic alteration in RedisDesktopManager~\cite{redisdesktopmanagercommit}. \mbox{"(-)"} indicates removed lines of code.}]
<qresource prefix="/">
        <file>translations/rdm_zh_CN.qm</file>
        <file>translations/rdm_zh_TW.qm</file>
(-)     <file>translations/rdm_ru_RU.qm</file>
        <file>translations/rdm_es_ES.qm</file>
        <file>translations/rdm_ja_JP.qm</file>
        <file>translations/rdm_uk_UA.qm</file>
    \end{lstlisting}
\end{figure}

% \textbf{Function Denial.} 
% \label{sec:funcdenial}
% A protestware has function denial if the code is altered to prevent further execution.
% We found examples of function denial through an infinite loop and removal of key functionality. 
% For instance, as shown in~\cref{colorsinfloop}, an infinite-loop was added to colors.js~\cite{colorscommit} to freeze the software and show the ASCII image in~\cref{colorsflag}. The modifications to colors.js was to protest large-corporations profiting off of free software without giving back~\cite{colorsnomorefreework}.

\begin{figure}[H]
    \centering
    \small 
    \begin{lstlisting}[style=base, 
        language=html, 
        label={colorsinfloop},
        caption={Example of function denial in colors.js.}]
let am = require('../lib/custom/american');
am();
for (let i = 666; i < Infinity; i++;) {...}
    \end{lstlisting}
\end{figure}


% \textbf{Temporal Proximity.} A protest exhibits temporal proximity if the publishing date of the protesting action is within 3 months of a newsworthy event (time requirement) and changes in the software relates to said event (relation requirement). 
% The relation between the changes in the software and the event can be determined by referring to one or more of the other symptoms.
% For example, Listings \ref{isofilt}, \ref{adcomm}, and \ref{redisnorustrans}, were all committed within 3 months of the start of the Russo-Ukrainian war and exhibit relation to Russia~\cite{awesomeprometheusalertscommit, esfiveextcommit, redisdesktopmanagercommit}.
% Furthermore, even if a commit does not explicitly mention an event, a protest can be inferred, \eg~\cite{yadcommit} dropped support for the Russian language (relation, also an example of linguisitic alteration) within 6 days of the start of the war (time). 
% The comments in~\cite{yadcommit} suggests that most would
% agree with our inference.


% \JC{End new prose. Below is old prose.}
% \begin{enumerate}
%     \item \textbf{Isolation Filter.} The source code performs some form of check that isolates a particular group of users, such as location, IP, or language checking, with the resulting behavior not being broadly applied to all groups, therefore making it not an accessibility feature.
%     \label{symptom:targetLocation}
    
%     \item \textbf{Advocacy Communication.} 
%     % \textbf{Activist Messaging.} 
%     The project contains one or more files (\eg code, documentation, images) with a message containing aggressive language or ideology promotion. This may or may not require the software to be run to be seen.
    
%     % \item \textbf{Aggressive Language.} The source code comments or additional writing (such as the README.md or licensing files) contains aggressive language and/or explicit political language. \label{symptom:aggressiveLanguage}
%     % \TF{Need to fix this as we aggregated this with the 4th symptom to include anything in the software, text, images, etc.}
    
%     \item \textbf{Linguistic Alteration.} The source code contains new string(s) in a language different than the primary language of the developer\footnote{Primary language is determined by the language of comments and text files like README.md. Also note that the strings should not be used for translation purposes}, or the developer removes a previously supported language entirely. 
%     \label{symptom:additionalLanguage}
    
%     % \item \textbf{Ideology Promotion.} The project contains an alteration of promotional content (things seen when the software is run) such as images or text to reflect some ideological beliefs. 
%     % \label{symptom:benign}
    
%     \item \textbf{Function Denial.} The code is altered to prevent further execution, typically through an infinite loop of some kind or removal of key functionality. 
%     \label{symptom:denail}

%     \item \textbf{Temporal Proximity.} The publishing date of the protesting action is close to ($\leq$ 3 months) a newsworthy event and changes in the software relates to said event.
%     \label{symptom:temporal}
    
% \end{enumerate}

% % Symptom ~\ref{symptom:targetLocation} is a fairly common practice among the protestware studied, especially the malicious ones. The idea is to detect if users come from a particular region before disallowing their access or performing additional malicious actions to their machine. The reason we specify a set smaller than accessibility feature is because a location or language check in the code could be performing different functionality depending on the region. However, the main distinction is the conditional behavior for only a specific region or language that is not accounted for (does not produce similar behavior) in other regions supported in the code. 

% % Symptom ~\ref{symptom:aggressiveLanguage} is the indication of the author to intend to prevent a group of people from accessing the functionality of their code because of emotional, personal, or political reasons. This symptom will fall under the public category if the text they insert is in a public and easily viewable file such as the README. Otherwise, the text may also be nested in a code file and inserted as comments on the functionality which would classify it as private. 

% % Symptom ~\ref{symptom:additionalLanguage} is an insight that many of the projects with protestware seem to be U.S. and English based, and exhibit strings of text to protest or communicate to their target audience (typically Russians). This should be distinguished from projects that have additional languages for functionality such as translation. Typically it is a message against the offending party which the developers are protesting in their native language of the offenders. The other option is to remove a regional language translation ability in order to protest against the offenders. Typically these projects will already offer translation capabilities for users, but remove a certain language in protest against that country/ users. 

% % Finally, symptom ~\ref{symptom:benign} is the least affecting to the code in terms of functionality. Most of these cases were isolated changes to the content of the repository displayed in promotional contexts.  


% %GPT's Improvmenet
% This is a prevalent practice among the studied protestware, in particular those categorized as malicious. Projects demonstrating this symptom will detect the user's region to restrict their access to that project or perform additional malicious actions on their machine. The reason we specify a smaller set of languages \JC{What do you mean by ``specifying'' a smaller set of languages?} rather than an accessibility feature is that a location or language check in the code could have different functionalities depending on the region. The main distinction lies in the conditional behavior specific to a certain region or language that is not replicated in other regions supported by the code. Figure ~\ref{fig:targetSymptom} shows an example of this symptom occurring in the repository of "es5-ext", where a conditional statement based on location is put in place to affect the behavior of the code without handling the other cases. 



% Symptom ~\ref{symptom:aggressiveLanguage} indicates the developer's intent to prevent a group of people from accessing their code's functionality \JC{It's unclear to me how aggressive language in README/licensing file can prevent access to code functionality. Or do you mean smth like ``DO NOT USE THIS CODE IF YOU'RE FROM COUNTRY X AND SUPPORT PRESIDENT ABC''?} due to emotional, personal, or political reasons. This symptom falls under the public category if the text is inserted in a public and easily viewable file, such as the README. Otherwise, the text may be nested in a code file and inserted as comments on the functionality, classifying it as private. Figure ~\ref{fig:aggressiveSymptom} shows an example of this symptom with aggressive language given when Russians are redirected to the HTML page shown\JC{Now I see what you mean. You deny usage by detecting their IP or smth (which is symptom 1) and then include a message (symption 2).}.



% Symptom ~\ref{symptom:additionalLanguage} reveals that many protestware projects seen were based in the U.S. and were English-centric, often containing text strings protesting or communicating with their target audience, typically utilizing Russian in this dataset as a result of the Russo-Ukrainian conflict ~\cite{dataset}. This should be distinguished from projects that offer additional languages for functionality, such as translation. Often, these messages are against the offending party in the developers' native language or involve removing a regional language translation ability to protest against the offenders. Some of these projects offer translation capabilities for users, but later, as a form of protest, remove a certain language. Figure ~\ref{fig:removeLangSymptom} shows an example of this symptom where the repository of "awesome-prometheus-alerts" removes the translation functionality for Russian, but not any other language previously supported. 



% Finally, symptom ~\ref{symptom:benign} has the least impact on the code's functionality. Most of these cases involve isolated changes to the repository's content displayed in promotional contexts. Figure ~\ref{fig:changeImage} shows a simple example of this symptom of the repository for "RedisDesktopManager" changing a background image. 

% \subsection{Stats}
% In~\cref{sympcounts}, we can see that \textbf{Temporal Proximity} had the most number of protestware due to 16 instances in the dataset relating to the start of the Russo-Ukraine war on Febuary 24, 2022. 
% Within two months, all 16 instances of protestware were realized. 
% The most recent instance of this symptom was the Israel-Hamas conflict around October 2023 and in the same month another instance of protestware was generated called 'e2eakarev'. 
% The remaining two instances did not have an associated event with them, thus showing the effectiveness of this symptom.
% We can see that the first three symptoms are fairly popular with about half\JC{Calculate exact amount} of the protestware having a manifestation of that symptom. The final symptom wasn't as popular with only 4 protestware exhibiting that symptom. \JC{May want to remind reader there are 16 total protestwares, so 4 means 25\%}

% \begin{figure} %Chart for symptoms, to give an overview of numbers
%     \centering
%     \includegraphics[width=\linewidth]{Figures/newSymptomChart.png}
%     \caption{ Bar chart of the number of occurences identified for each symptom across all protestware in our dataset. }
%     \label{fig:symptomChart}
% \end{figure}

% \begin{table}[h]
% \centering
% \caption{Symptom frequency. Note that the sum does not equal the number of protestware samples because a protestware may exhibit more than one symptom.
% \JC{TP\&IF=9, TP\&AC=8, TP\&LA=7, TP\&FD=1. Does this mean IF, AC, LA are all redundant symptoms and all we need is TP? Is there a case where TP return FP? Should we remove the ``related'' requirement from TP?}
% }
% \begin{tabular}{lr}
%  \toprule
% \textbf{Symptom} & \textbf{Count} \\
%  \toprule
% Temporal Proximity & 14 \\
% \hline
% Isolation Filter & 9 \\
% \hline
% Advocacy Communication & 8 \\
% \hline
% Linguistic Alteration & 7 \\
% \hline
% Function Denial & 3 \\
% \toprule
% Total altered software & 14 \\
% \toprule
% \end{tabular}
% \label{sympcounts}
% \end{table}


% Our final step was performing an inductive thematic analysis, which means we developed new classifications relative to discoveries found within the dataset of the 16 GitHub repositories, manually examining relevant commits provided by our source~\cite{dataset}. \JC{It's not clear from the methodology section how easy/hard or how much effort is needed to find such symptom by reviewing the commits. How many commits did you review? How long did it take? etc.} % It didn't take that long to find and review them, but most of the time was pulling a common theme.

% These commits are when the software was changed and had differences not typical of the original project and were analyzed to identify potential symptoms, where a symptom is an indicator of the attack type's presence. In the cases in which the commit was deleted entirely from the repository, or the repository itself was no longer accessible, the digital archive known as the Wayback Machine~\cite{Wayback} was utilized to access the commits directly for analysis. Upon gathering the symptoms for each repository individually, they were generalized to fit more cases than just the ones seen which enables the symptoms to better suit the development of detection tools. 

% Considering prior successful and documented attempts of protestware, this project will primarily focus on currently understood and categorized attack types, distinguishing between benign and malicious threats with a primary focus on the latter.  For the purposes of this study, following a thorough examination of preexisting documentation on both the current understanding of the attack type alongside previous reports regarding the vulnerabilities of open-source software, a dataset comprising of previously active forms of protestware contained within open-source software will be thoroughly examined to locate both utilized and potential points of security threat to any system that relies on them.  This will allow for both an understanding of the type of software that is often selected to be a carrier alongside an examination of emerging patterns related to what aspects of that software are typically modified during this type of attack. From this detail analysis, a set of criteria for flagging potential security risks can be constructed for the purposes of building a prototype for open-source program analysis that takes into account this new threat. 

% \subsection{Taxonomy Creation}
% \label{taxCreat}
% % \JC{Instead of taxonomy, maybe can just call these properties.}
% \JC{What the boys did: First found a paper that classified protestware into two categories~\cite{Protestware} mal and benign. Then they reviewed the collected protestware asynchronously. 
% One author suggested ``Target'' and another author suggested ``Visibility''. No one discussed any of these properties with each other, so maybe we should.
% }

% Firstly, through the development of a taxonomy through the examination of previous research and known documentation of occurrences of protestware in the media, a deductive thematic analysis was performed. \TF{I've been looking into it and it doesn't seem like we did a thematic analysis because it seems to require codebooks which we don't have. I think this was Sazz's suggestion, but I'm not sure how to integrate it. } This analysis is an examination of the dataset relative to the theoretical framework of classification we developed relative to the previous literature on the matter\JC{Find a paper that explains what `` deductive thematic analysis'' is and cite it} and examining the data relative to a set of defined categories for the attack vector, being its behavior, its target, and its visibility\JC{Sentence way too long. Rewrite.}. 
% % For each instance in the dataset, the relevant commit in the GitHub repository that introduced the protestware was analyzed \JC{How did you analyze it? Be specific.} to procure an understanding of which categories it fell under within the previously established framework\JC{Which previously established framework?}. % We didn't use the data set
% From the themes solidified by the coding process during the analysis, a taxonomy was developed \JC{What measure did you take to ensure that this taxonomy is valid? \ie why should we trust your taxonomy?} to encompass the possible variants of the attack vector alongside how those variants affect those utilizing the software, providing a framework for deeper analysis into the individual repositories themselves\JC{This section is for you to talk about how you created the taxonomy, not to sell its uses. Right now, the reader has no idea what you did to create the taxonomy.}.  

% \subsection{Symptomology Analysis}
% \label{sympt}
% Our final step was performing an inductive thematic analysis, which means we developed new classifications relative to discoveries found within the dataset of the 16 GitHub repositories, manually examining relevant commits provided by our source~\cite{dataset}. \JC{It's not clear from the methodology section how easy/hard or how much effort is needed to find such symptom by reviewing the commits. How many commits did you review? How long did it take? etc.} % It didn't take that long to find and review them, but most of the time was pulling a common theme.
% \JC{In case I forget, it is also possible that they added a potential symptom without specifying it in the commit, which is a limitation of this method. This is especially concerning for symption 1, since it involves the source code and reviewing the source code manually in its entirety would be infeasible. This comment should go in the threats to validity or limitation section.}
% These commits are when the software was changed and had differences not typical of the original project and were analyzed to identify potential symptoms, where a symptom is an indicator of the attack type's presence. In the cases in which the commit was deleted entirely from the repository, or the repository itself was no longer accessible, the digital archive known as the Wayback Machine~\cite{Wayback} was utilized to access the commits directly for analysis. Upon gathering the symptoms for each repository individually, they were generalized to fit more cases than just the ones seen which enables the symptoms to better suit the development of detection tools. Finally, an examination of the data surrounding the protestware in terms of the utilized programming language and popularity statistics, like number of forks and stars on the repositories, was performed, allowing an understanding of what type of project is more likely to be converted into protestware alongside how popularity has been seen and whether the popularity had changed after the insertion of protestware. In order to compare these statistics at the time of insertion of protestware, we also used the Wayback Machine to find the closest snapshot to the insertion and then another one about a week to a month after, depending on the frequency of snapshots provided. 

% Considering prior successful and documented attempts of protestware, this project will primarily focus on currently understood and categorized attack types, distinguishing between benign and malicious threats with a primary focus on the latter.  For the purposes of this study, following a thorough examination of preexisting documentation on both the current understanding of the attack type alongside previous reports regarding the vulnerabilities of open-source software, a dataset comprising of previously active forms of protestware contained within open-source software will be thoroughly examined to locate both utilized and potential points of security threat to any system that relies on them.  This will allow for both an understanding of the type of software that is often selected to be a carrier alongside an examination of emerging patterns related to what aspects of that software are typically modified during this type of attack. From this detail analysis, a set of criteria for flagging potential security risks can be constructed for the purposes of building a prototype for open-source program analysis that takes into account this new threat. 




==> results.tex <==
% \section{Results}

% This section discusses the results we collected, along with the analysis of results, and the generalizable symptoms which occur within the protestware we have seen. First, we use inductive reasoning to use a well known categorization scheme and see how it applies to the dataset of protestware. Then, we analyze the protestware with deductive reasoning to generate a set of symptoms, and we give a general discussion of the symptoms that typically occur within existing protestware. 

% Then, we evaluate specific types of protestware (based on our taxonomy) and how they relate to the symptoms that are produced as a possible way to identify these in conjunction or separate from any provided protestware. 
% These are all discussed in the context of the dataset of protestware projects collected and analyzed.


% \subsection{\textbf{RQ2}}

% After looking through all the protestware and applying deductive analysis on the set of features/patterns of the commits, the following set of symptoms was able to be derived through our manual analysis in order to answer \textbf{RQ2}:
%  \SR{At some place, we should acknowledge that by no means this is an exhaustive list of symptoms.}
% \begin{enumerate}
%     \item \textbf{Isolation Check} The source code performs some form of check that isolates a particular group of users, such as location, IP, or language checking, with the resulting behavior not being broadly applied to all groups, therefore making it not an accessibility feature.
   
%     \label{symptom:targetLocation}
%     \item \textbf{Aggressive Language} The source code comments or additional writing (such as the README.md or licensing files) contains aggressive language and/or explicit political language. \label{symptom:aggressiveLanguage}
%     \item \textbf{Language Barrier} The source code contains strings in a language different to the primary language of the developer\footnote{Primary language is determined by the language of comments and text files like README.md}, with those strings not being a part of a corpus of strings for language translation, or the developer removes a previously supported language entirely. \label{symptom:additionalLanguage}
%     \item \textbf{Promote Ideology} The project contains an alteration of promotional content (things seen when the software is run) such as images or text to reflect some ideological beliefs. \label{symptom:benign}
%     \item \textbf{Denial of Function} The code is altered to prevent further execution, typically through an infinite loop of some kind or removal of key functionality. \label{symptom:denail}
    
% \end{enumerate}

% % Symptom ~\ref{symptom:targetLocation} is a fairly common practice among the protestware studied, especially the malicious ones. The idea is to detect if users come from a particular region before disallowing their access or performing additional malicious actions to their machine. The reason we specify a set smaller than accessibility feature is because a location or language check in the code could be performing different functionality depending on the region. However, the main distinction is the conditional behavior for only a specific region or language that is not accounted for (does not produce similar behavior) in other regions supported in the code. 

% % Symptom ~\ref{symptom:aggressiveLanguage} is the indication of the author to intend to prevent a group of people from accessing the functionality of their code because of emotional, personal, or political reasons. This symptom will fall under the public category if the text they insert is in a public and easily viewable file such as the README. Otherwise, the text may also be nested in a code file and inserted as comments on the functionality which would classify it as private. 

% % Symptom ~\ref{symptom:additionalLanguage} is an insight that many of the projects with protestware seem to be U.S. and English based, and exhibit strings of text to protest or communicate to their target audience (typically Russians). This should be distinguished from projects that have additional languages for functionality such as translation. Typically it is a message against the offending party which the developers are protesting in their native language of the offenders. The other option is to remove a regional language translation ability in order to protest against the offenders. Typically these projects will already offer translation capabilities for users, but remove a certain language in protest against that country/ users. 

% % Finally, symptom ~\ref{symptom:benign} is the least affecting to the code in terms of functionality. Most of these cases were isolated changes to the content of the repository displayed in promotional contexts.  


% %GPT's Improvmenet
% Symptom ~\ref{symptom:targetLocation}\SR{Instead of using numbers, we should name the symptoms. For a reader, it is hard to map the symptoms with the number (revisiting the definitions each time is distracting).} is a prevalent \JC{Avoid adjectives, just say how many. ``Symptom 1 ocurred in 10 projects''.} practice among the studied protestware, in particular those categorized as malicious. Projects demonstrating this symptom will detect the user's region to restrict their access to that project or perform additional malicious actions on their machine. The reason we specify a smaller set of languages \JC{What do you mean by ``specifying'' a smaller set of languages?} rather than an accessibility feature is that a location or language check in the code could have different functionalities depending on the region. The main distinction lies in the conditional behavior specific to a certain region or language that is not replicated in other regions supported by the code. Figure ~\ref{fig:targetSymptom} shows an example of this symptom occurring in the repository of "es5-ext", where a conditional statement based on location is put in place to affect the behavior of the code without handling the other cases. 



% Symptom ~\ref{symptom:aggressiveLanguage} indicates the developer's intent to prevent a group of people from accessing their code's functionality \JC{It's unclear to me how aggressive language in README/licensing file can prevent access to code functionality. Or do you mean smth like ``DO NOT USE THIS CODE IF YOU'RE FROM COUNTRY X AND SUPPORT PRESIDENT ABC''?} due to emotional, personal, or political reasons. This symptom falls under the public category if the text is inserted in a public and easily viewable file, such as the README. Otherwise, the text may be nested in a code file and inserted as comments on the functionality, classifying it as private. Figure ~\ref{fig:aggressiveSymptom} shows an example of this symptom with aggressive language given when Russians are redirected to the HTML page shown\JC{Now I see what you mean. You deny usage by detecting their IP or smth (which is symptom 1) and then include a message (symption 2).}.



% Symptom ~\ref{symptom:additionalLanguage} reveals that many protestware projects seen were based in the U.S. and were English-centric, often containing text strings protesting or communicating with their target audience, typically utilizing Russian in this dataset as a result of the Russo-Ukrainian conflict ~\cite{dataset}. This should be distinguished from projects that offer additional languages for functionality, such as translation. Often, these messages are against the offending party in the developers' native language or involve removing a regional language translation ability to protest against the offenders. Some of these projects offer translation capabilities for users, but later, as a form of protest, remove a certain language. Figure ~\ref{fig:removeLangSymptom} shows an example of this symptom where the repository of "awesome-prometheus-alerts" removes the translation functionality for Russian, but not any other language previously supported. 
% \begin{figure*}
%     \centering
%     \small {
%     \begin{lstlisting}[language=Javascript]
% (+) if (
% (+)    [
% (+)        "Europe/Moscow", "Asia/Yakutsk", "Asia/Krasnoyarsk", "Europe/Samara",
% (+)        "Asia/Yekaterinburg", "Asia/Irkutsk", "Asia/Anadyr", "Asia/Kamchatka",
% (+)        "Europe/Kaliningrad", "Asia/Vladivostok", "Asia/Magadan", "Asia/Novosibirsk",
% (+)        "Asia/Omsk"
% (+)    ].indexOf(new Intl.DateTimeFormat().resolvedOptions().timeZone) === -1
% (+) ) {
% (+)    return;
% (+) }
%     \end{lstlisting}
%     }
%     % \includegraphics[width=\linewidth]{Figures/ScreenshotSymptom1.png}
%     \caption{ Example of Symptom 1 with a restriction based on a set of locations around Russia in a \href{https://github.com/medikoo/es5-ext/commit/28de285ed433b45113f01e4ce7c74e9a356b2af2}{commit} for repository es5-ext which is an extension to an existing library. A ``(+)'' indicates added code.}
%     \label{fig:targetSymptom}
% \end{figure*}

% \begin{figure*}
%     \centering
%     % \includegraphics[width=\linewidth]{Figures/ScreenshotSymptom2.png}
%     \small {
%     \begin{lstlisting}[language=html]
% File: [Middle finger emoji].md
% (+)<p>
% (+)    [Ukraine flag] Forbidden to Russian people.
% (+)    <br>
% (+)    <br>
% (+)    Please come back as soon as pease returns to Eastern Europe. [Ukraine flag] -
%        -[Handshake emoji] [Russian flag]
% (+)</p>
%     \end{lstlisting}
%     }
%     \caption{ Example of Symptom 2 with aggressive language against Russians in a \href{https://github.com/samber/awesome-prometheus-alerts/commit/6bfcdcca165e57c6fa09a561515c33284caa20c2}{commit} for a repository called 
% awesome-prometheus-alerts}
%     \label{fig:aggressiveSymptom}
% \end{figure*}

% \begin{figure}[h]
%     \centering
%     % \includegraphics[width=\linewidth]{Figures/ScreenshotSymptom3.png}
%     \small {
%     \begin{lstlisting}[language=html]
% <qresource prefix="/">
%         <file>translations/rdm_zh_CN.qm</file>
%         <file>translations/rdm_zh_TW.qm</file>
% (-)     <file>translations/rdm_ru_RU.qm</file>
%         <file>translations/rdm_es_ES.qm</file>
%         <file>translations/rdm_ja_JP.qm</file>
%         <file>translations/rdm_uk_UA.qm</file>
%     \end{lstlisting}
%     }
%     \caption{Example of Symptom 3 removing a Russian translation file for \href{https://github.com/RedisInsight/RedisDesktopManager/commit/8b2b357d9d233100f84a69f81ed22b8caa04fa22}{commit} in repository called RedisDesktopManager. \mbox{"(-)"} indicates removed lines of code. }
%     \label{fig:removeLangSymptom}
% \end{figure}

% Finally, symptom ~\ref{symptom:benign} has the least impact on the code's functionality. Most of these cases involve isolated changes to the repository's content displayed in promotional contexts. Figure ~\ref{fig:changeImage} shows a simple example of this symptom of the repository for "RedisDesktopManager" changing a background image. 

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\linewidth]{Figures/ScreenshotSymptom4.png}
%     \caption{Example of Symptom 4 where project called Evolution changes a background image to a political image with aggressive language against Russia in the \href{https://github.com/evolution-cms/evolution/commit/1c586bc76f739264dcf0482530945875fa444b77}{this commit}. }
%     \label{fig:changeImage}
% \end{figure}

% %I think this is already stated else where (May double check before delete)
% Next, we evaluated the protestware on our chosen category scheme. We have already seen that more benign than malicious protestware existed, and that some of the protestware we investigated were later removed, either as a commit to undo the changes or deleting the commit entirely. If it was the later case, we had to use a Wayback machine to access the code repositories in the state when protestware existed in them. Otherwise, the link to access the commit and repository were taken from the GitHub protestware dataset. 


% The dataset was then labeled with whether the symptoms we generated were occurring there. Figure ~\ref{fig:symptomChart} shows a bar chart of the number of protestware which had the a particular symptom. We can see that the first three symptoms are fairly popular with about half\JC{Calculate exact amount} of the protestware having a manifestation of that symptom. The final symptom wasn't as popular with only 4 protestware exhibiting that symptom. \JC{May want to remind reader there are 16 total protestwares, so 4 means 25\%}



==> tables/aftermath-stats.tex <==
% \newcommand{\posdiff}[1]{\textcolor{green!50!black}{#1}}
% \newcommand{\negdiff}[1]{\textcolor{red}{#1}}
% \newcommand{\neutraldiff}[1]{\textcolor{black}{#1}}

\begin{table*}[htbp]
\caption{Data of Protestware Popularity differences of altered software and altered documentation(bottom).}
% \SR{The number of projects are different from Table 1?}
% \JC{This is only for altered software}
\label{tab:aftermathStats}
\begin{tabular}{|l||r|r|r||r|r|r||r|r|r||
}
\hline
\textbf{Name} & \textbf{Prev. *} & \textbf{Stars} & \textbf{Diff} & \textbf{Prev. \frontaleye} & \textbf{Watch} & \textbf{Diff} & \textbf{Prev. Forks} & \textbf{Forks} & \textbf{Diff} \\
\hline
\hline
tasmota & 17200 & 21300 & \posdiff{24\%} & 655 & 631 & \negdiff{-4\%} & 3800 & 4700 & \posdiff{24\%} \\
\hline
APA & 3800 & 6000 & \posdiff{58\%} & 144 & 154 & \posdiff{7\%} & 653 & 942 & \posdiff{44\%} \\
\hline
node-ipc & 1000 & 41 & \negdiff{-96\%} & 21 & 3 & \negdiff{-86\%} & 126 & 7 & \negdiff{-94\%} \\
\hline
es5-ext & 135 & 166 & \posdiff{23\%} & 7 & 9 & \posdiff{29\%} & 49 & 81 & \posdiff{65\%} \\
\hline
EventSource & 1800 & 2100 & \posdiff{17\%} & 43 & 44 & \posdiff{2\%} & 299 & 330 & \posdiff{10\%} \\
\hline
Evolution & 259 & 262 & \posdiff{1\%} & 35 & 34 & \negdiff{-3\%} & 237 & 98 & \negdiff{-59\%} \\
\hline
voicybot & 750 & 881 & \posdiff{17\%} & 27 & 29 & \posdiff{7\%} & 117 & 161 & \posdiff{38\%} \\
\hline
SweetAlert2 & 14400 & 16800 & \posdiff{17\%} & 213 & 216 & \posdiff{1\%} & 1400 & 1600 & \posdiff{14\%} \\
\hline
Quake3e & 815 & 1100 & \posdiff{35\%} & 44 & 50 & \posdiff{14\%} & 93 & 143 & \posdiff{54\%} \\
\hline
RDM & 21100 & 22700 & \posdiff{8\%} & 612 & 627 & \posdiff{2\%} & 3200 & 3300 & \posdiff{3\%} \\
\hline
Qalculate & 450 & 887 & \posdiff{97\%} & 15 & 21 & \posdiff{40\%} & 35 & 66 & \posdiff{89\%} \\
\hline
YAD & 502 & 627 & \posdiff{25\%} & 22 & 24 & \posdiff{9\%} & 38 & 52 & \posdiff{37\%} \\
\hline
colors & 5200 & 5200 & \neutraldiff{0\%} & 54 & 54 & \neutraldiff{0\%} & 448 & 448 & \neutraldiff{0\%} \\
\hline
faker & 1500 & 1600 & \posdiff{7\%} & 104 & 109 & \posdiff{5\%} & 703 & 744 & \posdiff{6\%} \\
\hline
SC & 36200 & 40100 & \posdiff{11\%} & 373 & 365 & \negdiff{-2\%} & 2300 & 2500 & \posdiff{9\%} \\
\hline
left-pad & 1102 & 1300 & \posdiff{18\%} & 25 & 23 & \negdiff{-8\%} & 126 & 132 & \posdiff{5\%} \\
\hline \hline 
yandex & 0 & 0 & \neutraldiff{N/A} & 0 & 2 & \neutraldiff{N/A} & 0 & 0 & \neutraldiff{N/A} \\
\hline
pnpm & 14800 & 27700 & \posdiff{87\%} & 102 & 139 & \posdiff{36\%} & 408 & 911 & \posdiff{123\%} \\
\hline
nestjs-pino & 567 & 1200 & \posdiff{112\%} & 2 & 4 & \posdiff{100\%} & 68 & 98 & \posdiff{44\%} \\
\hline
\end{tabular}
\end{table*}

==> threatmodel.tex <==
\section{Threat Model}

Considering the challenges presented by protestware towards open-source software, especially as the use of such software has become normalized in current infrastructure, the primary directive is to ensure the safety of any user or set of users that accesses or utilizes it.  As the adversary in this scenario holds complete control over the software being modified as either a developer or contributor, with limitless capabilities in terms of potential additions or reductions, the primary defenders would be the users utilizing the software alongside developed forms of assisted code analysis to locate and remove any potential security threats prior to implementation.  In turn, it is assumed that the end user is willing and able to access information regarding potential alterations to open-source software, and examine utilized dependencies in full when they are modified.  Further, it is assumed that the potential attacker has both a complete understanding of and complete control over the modified software and, as a result, potential control over any and all systems that implement said software as a result.  

==> timeline.tex <==
\section*{Timeline}

\begin{center}
\begin{tabular}{||c | c||} 
 \hline
 Date & Action Item Completed\\ [0.5ex] 
 \hline\hline
 Feb.  21 & Thorough Literature Review  \\ 
 \hline
 March 20 & Protestware Attribute Collection \\
 \hline
 April 3 &  Preliminary solutions\\
 \hline
 April 29 & Effective solutions finalized \\[1ex] 
 \hline
\end{tabular}
\end{center}

For each of the aforementioned tasks, the group members will attempt to divide the load equally

% Tentative timeline of the project, with each team member's contribution.
